Regularized OFU: an Efficient UCB Estimator forNon-linear Contextual Bandit

Balancing exploration and exploitation (EE) is a fundamental problem in contex-tual bandit. One powerful principle for EE trade-off isOptimism in Face of Uncer-tainty(OFU), in which the agent takes the action according to an upper confidencebound (UCB) of reward. OFU has achieved (near-)optimal regret bound for lin-ear/kernel contextual bandits. However, it is in general unknown how to deriveefficient and effective EE trade-off methods for non-linearcomplex tasks, suchas contextual bandit with deep neural network as the reward function. In thispaper, we propose a novel OFU algorithm namedregularized OFU(ROFU). InROFU, we measure the uncertainty of the reward by a differentiable function andcompute the upper confidence bound by solving a regularized optimization prob-lem. We prove that, for multi-armed bandit, kernel contextual bandit and neuraltangent kernel bandit, ROFU achieves (near-)optimal regret bounds with certainuncertainty measure, which theoretically justifies its effectiveness on EE trade-off.Importantly, ROFU admits a very efficient implementation with gradient-basedoptimizer, which easily extends to general deep neural network models beyondneural tangent kernel, in sharp contrast with previous OFU methods. The em-pirical evaluation demonstrates that ROFU works extremelywell for contextualbandits under various settings.

==> contents/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{code: https://github.com/submit21neurips/rofu}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> contents/ntkbandit-bak.tex <==

\section{Achieving $\tilde{O}(\sqrt{T})$ regret for neural network in the NTK regime}

The whole procedure is described in Algorithm \ref{alg:ntkROFU}.

\begin{algorithm}[htb!]
\caption{ROFU in NTK regime}
\label{alg:ntkROFU}  
\begin{algorithmic}[1]

\STATE \textbf{Input}: A reward function $f_{\theta}$ with unknown $\theta$, number of rounds $T$, regularization parameter $\lambda$, step sizes $\alpha, \beta$, number of gradient descent steps $G$, network width $m$ and network depth $L$. 
\STATE Random initialized parameter $\theta^{(0)}$ and let $\theta_0 = \theta^{(0)}$. 
\STATE $D_0:=\emptyset$. 
\FOR{t = 1, ..., T}

    \STATE Observe ${(x_{t}, a)}_{a\in A}$. $\forall a \in A$, compute
    % \STATE $\forall a \in A$, compute $\hat{\theta}(x_{t},a) = \text{UPDATE}(x_t, a, \theta^{(0) },D_{t-1}, \alpha)$ and $\text{OFU}^{R}(x_{t},a) : = f_{\theta_{t-1}}(x_t, a) + g(f_{\hat{\theta}(x_t,a)}(x_t, a)- f_{\theta_{t-1}}(x_t, a))$
    % \STATE  
    \begin{flalign}
    &\hat{\theta}(x_{t},a) = \text{UPDATE}(x_t, a, \theta^{(0) },D_{t-1}, \alpha), \\
    &\text{OFU}^{R}(x_{t},a) : = f_{\theta_{t-1}}(x_t, a) + g(f_{\hat{\theta}(x_t,a)}(x_t, a)- f_{\theta_{t-1}}(x_t, a))
    \end{flalign}%$\hat{\theta}(x_{t},a) = \text{UPDATE}(x_t, a, \theta^{(0) },D_{t-1}, \alpha)$ and $\text{OFU}^{R}(x_{t},a) : = f_{\theta_{t-1}}(x_t, a) + g(f_{\hat{\theta}(x_t,a)}(x_t, a)- f_{\theta_{t-1}}(x_t, a))$
    
    \STATE Take $a_t = \argmax_{a\in A} \text{OFU}^{R}(x_t,a)$ and receive reward $r_t$. Let $D_t := D_{t-1}\cup \{(x_t, a_t, r_t)\}$.
    

    \STATE Let $\theta_t$ = TrainNN($D_t, \beta, \theta^{(0)}$).
\ENDFOR 
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[t]
% \caption{UPDATE($x_t, a, \bar{\theta}, D, \alpha$)}
% \label{alg:ntkupdate}  
% \begin{algorithmic}[1]
% \STATE Define $\mathcal{L}(\theta, D, \bar{\theta}) = \frac{1}{2}\left[\sum_{(x,a,r)\in D} (f(x,a; \theta)-r)^2 +\lambda \|\theta-\bar{\theta}\|^2\right]$


% \FOR{i=0, ..., I-1}

%     \STATE $\theta^{(i+1)} = \theta^{(i)} + \alpha [\nabla_\theta f(x_t, a; \theta^{(i)}) - \eta \nabla \mathcal{L}(\theta^{(i)})]$.
% \ENDFOR
% \STATE \textbf{RETURN} $\theta^{(I)}$. 
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}[t]
\caption{TrainNN($D, \beta, \bar{\theta}$)}
\label{alg:ntktrainNN}  
\begin{algorithmic}[1]
\STATE Define $\mathcal{L}(\theta, D, \bar{\theta}) = \frac{1}{2}\left[\sum_{(x,a,r)\in D} (f(x,a; \theta)-r)^2 +\lambda \|\theta-\bar{\theta}\|^2\right]$

\FOR{j=0, ..., J-1}

    \STATE $\theta^{(j+1)} = \theta^{(j)} - \beta \nabla \mathcal{L}(\theta^{(j)})$.
\ENDFOR
\STATE \textbf{RETURN} $\theta^{(J)}$. 

\end{algorithmic}
\end{algorithm}

The $\text{UPDATE}$ procedure is given by 
\begin{flalign}
\hat{\theta}(x_{t},a) = \argmax \tilde{f}_{\theta}(x_t,a;\theta_{t-1}) + \eta \tilde{\gL}(\theta, D_{t-1};\theta_{t-1}), 
\end{flalign}
where $\tilde{f}_{\theta}(x_t,a;\theta_{t-1})=f_{\theta_{t-1}}(x_t,a) + \langle g_{\theta_{t-1}}(x_t,a),\theta -\theta_{t-1}\rangle$ is the first order Taylor expansion of $f_{\theta}(x_t,a)$ at $\theta_{t-1}$ and $\tilde{\gL}(\theta, D_{t-1};\theta_{t-1}) :=\sum_{(x,a,r)\in D_{t-1}} (f_{\theta_{t-1}}(x,a) + \langle g_{\theta_{t-1}}(x,a),\theta -\theta_{t-1}\rangle -r)^2 + \lambda \|\theta- \theta^{(0)}\|^2$  is the first order Taylor expansion of $\tilde{\gL}(\theta, D_{t-1})$ at $\theta_{t-1}$.

The theoretical guarantee would be like the following. We abuse the notation $A$ to denote the set of action and its cardinality, which should be clear by itself within a context.

\begin{Thm}
If the network width satisfies $m\ge \text{poly}(T,A, L, \lambda^{-1}, \lambda_0^{-1})$ and the learning rates $\alpha, \beta \le C(mTL+m\lambda)^{-1}$, then with probability at least $1-\delta$, the regret of Algorithm 1 satisfies that 
\begin{flalign}
R_T \le \tilde{O}(\sqrt{T}\times \sqrt{\tilde{d}}),
\end{flalign}
where the $\hat{d}$ is the effective dimension and defined as 
\begin{flalign}
\tilde{d} = \frac{\log \det (\mI +\mH/\lambda)}{\log (1+TA/\lambda)}.
\end{flalign}
\end{Thm}

For the proof, we first analyze the following procedure. Suppose that the all the iterates are in the local neighborhood near the initialization. Moreover, we have the Taylor approximation in the neighborhood.
\begin{Lem}[Lemma 4.1\& Theorem B.3, \cite{cao2019generalization}]\label{lem:first-order-approx}
There exist constants $c_1,c_2,c_3>0$ such that for any $\delta\in(0,1)$, if $\omega$ satisfies that $c_1 (mL)^{-3/2}\left(\log (TAL^2/\delta)\right)^{3/2} \le \omega \le c_2 L^{-6} (log m)^{-3/2}$, then with probability at least $1-\delta$, for all $\theta, \tilde{\theta}$ with $\|\tilde{\theta}-\theta_0\|_2 \le \omega, \|\theta-\theta_0\|_2 \le \omega$, and all $j\in [TA]$ we have 
\begin{flalign}
&\left|f(x^j; \tilde{\theta}) -f(x^j;\theta) - \langle g(x^j;\theta),  \tilde{\theta} - \theta \rangle\right| \le c_3 \omega^{4/3} L^3 \sqrt{m\log m},\\
&\|g(x^j;\theta)\|_F \le c_4 \sqrt{mL}.
\end{flalign}
\end{Lem}

\begin{Lem}[Theorem 5, \cite{allen2019convergence}] \label{lem:gradient-distance}
There exist constants $c_1,c_2,c_3>0$ such that for any $\delta \in (0,1)$, if $\omega$ satisfies that $c_1 (mL)^{-3/2}\max\{\log^{-3/2} m, \log^{3/2} (TA/\delta)\}\le \omega \le c_2 L^{-9/2} \log^{-3} m\} \le \omega \le c_2 L^{-6} (log m)^{-3/2}$, then with probability at least $1-\delta$, for all $\theta$ with $\|\theta-\theta_0\|_2 \le \omega$, and for all $j\in [TA]$ we have 
\begin{flalign}
\|g(x^j;\theta)-g(x^j;\theta_0)\|_2 \le c_3 \sqrt{\log m}\omega^{1/3}L^3 \|g(x^j;\theta_0)\|_2. 
\end{flalign}
\end{Lem}

With these results, we can estimate the $\hat{\theta}(x_t,a)$ as follows.

To derive the NeuralUCB result \cite{zhou2020neural}, we choose the regularizer to be the following
\begin{flalign}
 \mathcal{L}(\theta, D_{t-1}) = \sum_{(x,a,r)\in D_{t-1}} (f(x,a;\theta_{t-1}) + \langle g_{\theta_{t-1}}(x,a),\theta -\theta_{t-1}\rangle -r)^2 + \lambda \|\theta- \theta_{t-1}\|^2
\end{flalign}
It is a first-order Taylor expansion of the regression objective at $\theta_{t-1}$.

To study the subroutine $\text{UPDATE}(x_t,a, \theta_{t-1}, D_{t-1}, \alpha)$, we consider the following problem
\begin{flalign}
\hat{\theta}(x_t ,a) = \argmin_\theta \tilde{f}(x_t,a, \theta_{t-1};\theta) +\eta \left(\sum_{(x,a,r)\in D_{t-1}}(f_\theta (x,a)-r)^2 +\lambda \|\theta -\theta_{t-1}\|^2\right), \label{eq:neuralUCB-update}
\end{flalign}
where $\tilde{f}(x_t,a, \theta_{t-1};\theta) = f(x_t,a;\theta_{t-1}) + \langle g_{\theta_{t-1}}(x_t,a),\theta -\theta_{t-1}\rangle$.

We will show near the $\theta_{t-1}$, we have
\begin{flalign}
f(x_t,a;\theta) \approx \tilde{f}(x_t,a,\theta_{t-1};\theta).
\end{flalign}

Hence, we have 
\begin{flalign}
\frac{\partial \gL}{\partial \theta } =& \sum_{(x,a,r)\in D_{t-1}} (f(x,a;\theta_{t-1}) -r) g_{\theta_{t-1}}(x,a) + \lambda (\theta_{t-1}-   \theta^{(0)}) \\
&+ \sum_{(x,a,r)\in D_{t-1}} \langle g_{\theta_{t-1}}(x,a),\theta -\theta_{t-1}\rangle g_{\theta_{t-1}}(x,a) + \lambda (\theta - \theta_{t-1}).
\end{flalign}
We assume  $\sum_{(x,a,r)\in D_{t-1}} (f(x,a;\theta_{t-1}) -r) g_{\theta_{t-1}}(x,a) + \lambda (\theta_{t-1}-   \theta^{(0)}) =0$ due to the first-order condition of optimality and that $\theta_{t-1}$ should minimize the regression objective.

The solver $\hat{\theta}(x_t,a)$ to problem (\ref{eq:neuralUCB-update}) must satisfy the first-order  condition for optimality: 
\begin{flalign}
g_{\theta_{t-1}}(x_t,a) - \eta \left[ \sum_{(x,a,r) \in D_{t-1}}\langle g_{\theta_{t-1}}(x,a), \theta - \theta_{t-1}\rangle g_{\theta_{t-1}}(x,a) + \lambda (\theta - \theta_{t-1})\right] = 0. %\Large|_{\theta=\hat{\theta}(x_t,a)}
\end{flalign}
% That is 
% \begin{flalign}
% \frac{1}{\eta} g_{\theta_{t-1}}(x_t,a) - \left[ \sum_{(x,a,r) \in D_{t-1}} g_{\theta_{t-1}}(x,a) g_{\theta_{t-1}}(x,a)^T+\lambda \mI\right](\theta - \theta_{t-1}) = 0.
% \end{flalign}
Solving the above equation for $\theta$, we obtain $$\hat{\theta} = \theta_{t-1} +\frac{1}{2\eta}\left[ \sum_{(x,a,r) \in D_{t-1}} g_{\theta_{t-1}}(x,a) g_{\theta_{t-1}}(x,a)^T+\lambda \mI\right]^{-1} g_{\theta_{t-1}}(x_t,a). $$


Furthermore, we substitute this $\hat{\theta}$ into the $\text{OFU}^{R}(x_t,a)$ formula and obtain
\begin{flalign}
 &\text{OFU}^{R}(x_t,a)= f(x_t,a;\theta_{t-1}) + \sqrt{f(x_t,a; \hat{\theta}(x_t,a)) - f(x_t,a; \theta_{t-1})}\\
&= f(x_t,a;\theta_{t-1}) + \sqrt{ g_{\theta_{t-1}}(x_t,a)^T\left[ \sum_{(x,a,r) \in D_{t-1}} g_{\theta_{t-1}}(x,a) g_{\theta_{t-1}}(x,a)^T+\lambda \mI\right]^{-1} g_{\theta_{t-1}}(x_t,a) }
\end{flalign}
This is close to the NeuralUCB formula.

We modify the objective of the procedure $\text{UPDATE}(x_t,a,\bar{\theta}, D, \alpha)$.
We use the first order Taylor expansion of $f(x_t,a)$ at point $\theta_{t-1}$ in the objective. Now the new objective becomes 
\begin{flalign}
V(\theta; &\theta_{t-1}) := \left[f_{\theta_{t-1}}(x_t,a) + \langle g_{\theta_{t-1}}(x_t,a),\theta -\theta_{t-1}\rangle\right] \nonumber\\
& + \eta\left[\sum_{(x,a,r)\in D_{t-1}} (f_{\theta_{t-1}}(x,a) + \langle g_{\theta_{t-1}}(x,a),\theta -\theta_{t-1}\rangle -r)^2 + \lambda \|\theta- \theta^{(0)}\|^2\right].
\end{flalign}


\begin{flalign}
V(\theta; &\theta_{t-1}) := \left[f_{\theta_{t-1}}(x_t,a) + \langle g_{\theta_{t-1}}(x_t,a),\theta -\theta_{t-1}\rangle\right] \nonumber\\
& + \eta\left[\sum_{(x,a,r)\in D_{t-1}} (f_{\theta_{t-1}}(x,a) + \langle g_{\theta_{t-1}}(x,a),\theta -\theta_{t-1}\rangle -r)^2 + \lambda \|\theta- \theta^{(0)}\|^2\right].
\end{flalign}

We introduce a notation $V(\theta; \theta_{t-1}) :=  \tilde{f}_{\theta}(x_t,a;\theta_{t-1}) + \eta \tilde{\gL}(\theta, D_{t-1};\theta_{t-1})$, and then $\hat{\theta}(x_t,a) = \argmax_\theta V(\theta; \theta_{t-1})$.
This problem is equivalent to a constrained optimization for some $\gamma_t$
\begin{flalign}
\argmax_{\theta: \tilde{\gL}(\theta, D_{t-1};\theta_{t-1}) \le \gamma_t}  \langle g_{\theta_{t-1}}(x_t,a),\theta -\theta_{t-1}\rangle.
\end{flalign}
Moreover, the constraint $\tilde{\gL}(\theta, D_{t-1};\theta_{t-1}) \le \gamma_t$  is equivalent to the following ellipsoid constraint
\begin{flalign}
\|\theta - \theta_{t-1}\|_{\mZ_{t-1}} \le \tilde{\gamma}_t,
\end{flalign}
where $\mZ_{t-1} := \lambda \mI + \sum_{(x,a,r)\in D_{t-1}} g_{\theta_{t-1}}(x,a)g_{\theta_{t-1}}(x,a)^T$ by assuming that $\theta_{t-1}$ satisfies the first-order optimality condition of minimizing the $\gL(\theta;D_{t-1})$. 

We note that 
\begin{flalign}
\langle g_{\theta_{t-1}}(x_t,a),\hat{\theta}(x_t,a) -\theta_{t-1}\rangle &= \max_{\theta: \|\theta - \theta_{t-1}\|_{\mZ_{t-1}} \le \tilde{\gamma}_t} \langle g_{\theta_{t-1}}(x_t,a),\theta -\theta_{t-1}\rangle\\
& = \tilde{\gamma}_t\sqrt{g_{\theta_{t-1}}(x_t,a)^T \mZ_{t-1}^{-1} g_{\theta_{t-1}}(x_t,a)}.
\end{flalign}


Hence if we choose $\eta =1$ and the function $g(x) = x$, then the $\text{OFU}^{R}$ becomes
\begin{flalign}
\text{OFU}^{R}(x_t,a) = f_{\hat{\theta}(x_t,a)} (x_t,a).
\end{flalign}

We know that the first order Taylor expansion gives 
\begin{flalign}
\text{OFU}^{R}(x_t,a) &= f_{\hat{\theta}(x_t,a)} (x_t,a) \nonumber \\ &\approx f_{\theta_{t-1}}(x_t,a) +\langle g_{\theta_{t-1}}(x_t,a),\hat{\theta}(x_t,a) -\theta_{t-1}\rangle \nonumber \\
&= f_{\theta_{t-1}}(x_t,a) +  \tilde{\gamma}_t\sqrt{g_{\theta_{t-1}}(x_t,a)^T \mZ_{t-1}^{-1} g_{\theta_{t-1}}(x_t,a)}.
\end{flalign}

This is almost the same as the $U_{t,a}$ in Algorithm 1 (NeuralUCB) in \cite{zhou2020neural}. One difference is that \citep{zhou2020neural} use  $\tilde{\mZ}_t := \lambda \mI + \sum_{\tau=1}^t g_{\theta_{\tau-1}}(x_\tau,a_\tau) g_{\theta_{\tau-1}}(x_\tau,a_\tau)^T$.

We next show that $\mZ_t$ enjoys the same property as $\tilde{\mZ}_t$ as follows. We introduce another sequence $\bar{\mZ}_t = \lambda \mI + \frac{1}{m} \sum_{\tau =1}^t g_{\theta_0}(x_\tau,a_\tau)g_{\theta_0}(x_\tau, a_\tau)^T$.
\begin{Lem}[Lemma B.3 in \cite{zhou2020neural}]
With probabililty $1-\delta$ where $\delta\in (0,1)$, for any $t\in [T]$, we have 
\begin{flalign}
\|\mZ_t\|_2 \le \lambda + c_1 t L, \quad \|\mZ_t -\bar{\mZ}_t\|_F \le c_2 m^{-1/6} \sqrt{\log m} L^4 t^{7/6} \lambda^{-1/6},
\end{flalign}
if the network width $m$ satisfies that
\begin{flalign}
c_3 m^{-3/2} L^{-3/2}[\log (TKL^2/\delta)]^{3/2} \le 2 \sqrt{t/(m\lambda)} \le c_4 L^{-6} [\log m]^{-3/2}, \forall t \in [T],
\end{flalign}
with some constants $c_1,c_2, c_3, c_4>0$.
\end{Lem}
\begin{proof}
The proof can be adapted from that of Lemma B.3 in \cite{zhou2020neural} with the fact that $\|g_{\theta_{t-1}}(x,a) - g_{\theta_0}(x,a)\|_2$ is bounded from the above because of Lemma \ref{lem:gradient-distance}.
\end{proof}

Hence we can establish a similar result as Lemma 5.2 in \cite{zhou2020neural} that with high probability, the optimal $\theta^*$ lies in the sequence of confidence sets, i.e., an ellipsoid defined with the new  matrix $\mZ_t$.

Next, in order to prove a similar result as Lemma 5.3 in \cite{zhou2020neural}, we only need to bound 
\begin{flalign}
|\text{OFU}^R(x_t,a) - \tilde{U}_{t,a}|,
\end{flalign}
where $\tilde{U}_{t,a} := \langle g_{\theta_{t-1}}(x_t,a),\theta_{t-1}-\theta_0\rangle + \gamma_{t-1} \sqrt{g_{\theta_{t-1}}(x_t,a)^T \mZ_{t-1}^{-1} g_{\theta_{t-1}}(x_t,a)/m}$.
The derivation is as follows,
\begin{flalign}
|\text{OFU}^R(x_t,a) - \tilde{U}_{t,a}| &\le |\text{OFU}^R(x_t,a)- f_{\theta_{t-1}}(x_t,a) -  \tilde{\gamma}_t\sqrt{g_{\theta_{t-1}}(x_t,a)^T \mZ_{t-1}^{-1} g_{\theta_{t-1}}(x_t,a)}| \nonumber\\
&\quad+ |f_{\theta_{t-1}}(x_t,a)+\tilde{\gamma}_t\sqrt{g_{\theta_{t-1}}(x_t,a)^T \mZ_{t-1}^{-1} g_{\theta_{t-1}}(x_t,a)}- \tilde{U}_{t,a}|\nonumber\\
&= |f_{\hat{\theta}(x_t,a)}(x_t,a) - f_{\theta_{t-1}}(x_t,a) -  \langle g_{\theta_{t-1}}(x_t,a),\hat{\theta}(x_t,a) -\theta_{t-1}\rangle| \nonumber\\
&\quad + |f_{\theta_{t-1}}(x_t,a) - f_{\theta_{0}}(x_t,a) - \langle g_{\theta_{t-1}}(x_t,a),\theta_{t-1}-\theta_0\rangle| \\
& \le 2c_3 m^{-1/6} \sqrt{\log m} t^{2/3} \lambda^{-2/3} L^3,
\end{flalign}
where $c_3$ is a constant and the last inequality is due to Lemma \ref{lem:first-order-approx}. Hence we show the $\text{OFU}^R(x_t,a)$ shares the same property as the $U_{t,a}$ in Algorithm 1 of \cite{zhou2020neural}. The left proof follows a similar procedure.
